Enhancing GNNs Performance on Combinatorial Optimization by Recurrent Feature Update

Combinatorial optimization (CO) problems are crucial in various scientific and industrial applications. Recently, researchers have proposed using unsupervised Graph Neural Networks (GNNs) to address NP-hard combinatorial optimization problems, which can be reformulated as Quadratic Unconstrained Binary Optimization (QUBO) problems. GNNs have demonstrated high performance with nearly linear scalability and significantly outperformed classic heuristic-based algorithms in terms of computational efficiency on large-scale problems. However, when utilizing standard node features, GNNs tend to get trapped to suboptimal local minima of the energy landscape, resulting in low quality solutions. We introduce a novel algorithm, denoted hereafter as QRF-GNN, leveraging the power of GNNs to efficiently solve CO problems with QUBO formulation. It relies on unsupervised learning by minimizing the loss function derived from QUBO relaxation. The proposed key components of the architecture include the recurrent use of intermediate GNN predictions, parallel convolutional layers and combination of static node features as input. Altogether, it helps to adapt the intermediate solution candidate to minimize QUBO-based loss function, taking into account not only static graph features, but also intermediate predictions treated as dynamic, i.e. iteratively changing recurrent features. The performance of the proposed algorithm has been evaluated on the canonical benchmark datasets for maximum cut, graph coloring and maximum independent set problems. Results of experiments show that QRF-GNN drastically surpasses existing learning-based approaches and is comparable to the state-of-the-art conventional heuristics, improving their scalability on large instances.

==> background.tex <==


\\ \\
\textbf{GraphSAGE \& LSTM aggregator}.
GraphSAGE is a general inductive framework that leverages node feature information to efficiently generate node embeddings
by sampling and aggregating features from a node’s local neighborhood.

%There are many different types of specific message-passing protocols that can be used \cite{hamilton2017allconv}.
%The architecture of QRF-GNN is based on the GraphSAGE framework \cite{hamilton2017sage}.
In the case of GraphSAGE the feature vector for each node $i$ aggregates information about a node's local neighborhood $N(i)$ and receives an update according to the following scheme:
\begin{equation}
    \label{eq:sage_layer}
    \begin{split}
       & h^{l+1}_{N(i)} = \rho  \left( \left\{ h^l_j, \forall j \in N(i) \right\} \right), \\
       & h^{l+1}_i = f \left( W^l \big[h^l_i \ h^{l+1}_{N(i)}\big] \right),
    \end{split}
\end{equation}
where $f$ is a nonlinearity function and $W^l$ is a matrix of trainable parameters acting on concatenated vectors $h^l_i$ and $h^{l+1}_{N(i)}$.
The size of the matrix $W^l$ depends on the dimension of input vectors and the given size of hidden states.
Different aggregation methods $\rho$, such as averaging, pooling or LSTMs~\cite{hamilton2017sage}, can be adopted here.
Recurrence is used here only in the sense that LSTM aggregators process feature vectors of node's neighbors as a sequence
without having any information about their states at the previous iteration.
\\ \\
\textbf{RUN-CSP}.
The RUN-CSP architecture is aimed at finding approximate solutions for any binary maximum constraint satisfaction (Max-CSP) problem.
A message passing protocol of the used GNN is executed on a graph with nodes for all variables of the instance and edges for all constraints.
During message passing all variables $x, y$ that co-occur in a constraint $c=(x, y, R)$ with a relation $R$ exchange messages.
A short-term state vector $s^{(t)} \in \mathbb{R}^{k}$ and a hidden (long-term) state vector $h^{(t)} \in \mathbb{R}^{k}$ are associated with every variable.
For every relation $R$ a trainable matrix is defined and applied to stacked $2k$-dimensional vector consists of $s^{(t)}_x$ and $s^{(t)}_y$ to generate a stacked vector of messages $m_{x,i}, m_{y,i}$.
After the message passing step current states as well as internal long-term states are updated by an LSTM cell:
\begin{equation}
    h^{(t + 1)}_x, s^{(t + 1)}_x = \text{LSTM}\left( h^{(t)}_x, s^{(t)}_x, \frac{1}{l}\sum_{i=1}^{l}m_{x,i}  \right).
\end{equation}
For every step $t$ a variable assignment in a search domain is calculated as $\phi^{(t)}(x) = \text{softmax}(Ws^{(t)}_x)$.
Then the objective function for a particular instance is combined throughout given number of iterations $t_{\max}$ with discount factor $\lambda \in [0,1]$:
\begin{equation}
    \begin{split}
        &\mathcal{L}:=\sum_{t=1}^{t_{\max}}\lambda^{t_{\max} - t} \cdot \mathcal{L}_{\text{CSP}}(\phi^{(t)}), \\
        &\mathcal{L}_{\text{CSP}}(\phi^{t}):= \frac{1}{|C|} \cdot \sum_{(x, y, R) \in C} - \log(\phi^{(t)}(x)^TA_R\phi^{(t)}(y)),
    \end{split}
\end{equation}
where $A_R$ is a characteristic matrix of the relation $R$ with $(A_R)_{i,j}=1$ if $(i, j) \in R$, and $C$ is a set of constraints $(x, y, R)$.
Thus, at each epoch the fixed number of iterations is computed and then the cumulative loss function is minimized, after which the states are reinitialized.

%\[
%        {SR(s_x^{(t)}, s_y^{(t)})}= MR\begin{pmatrix}s_x^{(t)} \\ s_y^{(t)}\end{pmatrix}
%\]
%
%or
%
%\[
%        {SR(s_x^{(t)}, s_y^{(t)})} = \left(  MR\begin{pmatrix}s_x^{(t)} \\ s_y^{(t)}\end{pmatrix}, MR\begin{pmatrix}s_y^{(t)} \\ s_x^{(t)}\end{pmatrix}\right),
%\]
%
%where in the first case $MR \in \mathbf{R}^{2k\times 2k}$ and in the second $MR \in \mathbf{R}^{2k\times k}$ depending on whether relations are asymmetric or symmetric.


%Based on the output, the network produces probabilities of a variable taking a certain value in the search domain.

==> experiments2.tex <==
During experiments, we found out that there was no need to do a time-consuming optimization of hyperparameters (as it is done in the PI-GNN algorithm) to overcome existing GNNs.
However, the hyperparameters tuning may lead to better results of QRF-GNN.
The only parameters that we changed were the size of hidden layers and the maximum number of iterations, since for some types of graphs fewer iterations were sufficient to get a competitive result.
We limited the number of iterations to $5 \times 10^4$ for random regular graphs and $10^5$ for all the other graphs, but in some cases convergence was reached much earlier.
If the value of the loss function at the last 500 iterations had differed by less than $10^{-5}$ it was decided that the convergence was achieved and the training was stopped. %or the current best value does not change for more than $10^4$ iterations
In the case of the graph coloring problem, an additional stopping criterion was used and the solution was considered to be found when the absolute value of the loss function becomes less than $10^{-3}$.
The learning rate was set empirically to 0.014 for the Adam optimizer, leaving the remaining parameters unaltered.
The dropout was set to 0.5.
The dimension of the random part of input vectors was equal to 10, the size of hidden layers was fixed at 50 for Max-Cut and at 140 for graph coloring.
\
Due to the stochasticity of the algorithm, it is preferable to do multiple runs with different seeds to find the best result.
One can do separate runs in parallel possibly utilizing several GPUs.
If the device has enough memory, the RUN-CSP scheme by \cite{Tonshoff2021} can be used.
In this case, one composite graph with duplicates of the original one is created for the input.
We trained the model in parallel on the NVIDIA Tesla V100 GPU.
Conventional heuristics were launched on the machine with two Intel Xeon E5-2670 v3 @ 2.30GHz.
The computational time depended on the size of the graph and the achievement of convergence, but the longest run of QRF-GNN did not exceed 17 minutes.

\subsection{Max-cut}\label{subsec:maxcut}
%
%Max-Cut is a classic well-known combinatorial problem, which is to divide the vertices of the graph $\gG=(\gV, \gE)$ into two subsets such
%that the number of edges whose adjacent nodes are in different subsets is maximum (or the total weight of such edges in the case of a weighted graph).
%Its QUBO formulation is as follows:
%
%\begin{equation}
% \label{eq:qubo-maxcut}
%  \begin{split}
%  &\max \quad \frac{1}{2} \sum_{i<j} w_{ij} (1 - x_i x_j), \\
%  &\text{ s.t.} \quad x_i \in \left\{ 0, 1 \right\}, \quad \forall i \in \gV.
%  \end{split}
%\end{equation}
%
%\noindent where $w_{ij}$ is the weight of the edge $(i, j)$  in the graph $\gG$.
%In this paper we consider only unweighted graphs with $w_{ij}=1$,~$ \forall (i,j) \in \gE$.
%
%The objective function \ref{eq:qubo-maxcut} can be rewritten as follows:
%%in a more physics-inspired \cite{Schuetz2022} way as
%
%\begin{equation}
% \label{eq:qubo-maxcut-xQx}
%  F_\text{QUBO} = \mathbf{x}^{T} Q \mathbf{x} = \sum_{i,j} x_i Q_{ij} x_j, \quad Q = A - D,
%\end{equation}
%
%\noindent where $A$ is an adjacency matrix of the graph and $D$ is a diagonal matrix with degrees of corresponding nodes.

To evaluate the performance of QRF-GNN, we compared results with other GNNs and popular heuristics on several datasets.


Table \ref{table:res-maxcut-dreg} shows the mean \emph{P-value}~$=\sqrt{\frac{4}{d}} \left(\frac{z}{n} - \frac{d}{4} \right)$ obtained with extremal optimization heuristics (EO) by \cite{Boettcher2003}, RUN-CSP and QRF-GNN
for random regular graphs with $n=500$ nodes and different degrees $d$.
Here $z$ corresponds to the obtained cut size.
Results of EO and RUN-CSP were taken from \cite{Tonshoff2021}, where \emph{P-value} was averaged over 1000 graphs.
RUN-CSP was allowed to make 64 runs for each graph and in the case of EO the best of two runs was chosen \cite{Yao2019}.
\emph{P-values} of PI-GNN depend on the particular architecture.
Results for graphs with a degree 3 and 5 were published in   \cite{Schuetz2022} for the architecture with GCN layer, and it corresponds to the first value in the column for PI-GNN.
The cut size was bootstrap-averaged over 20 random graph instances and PI-GNN took up to 5 shots.
In the paper by \cite{Schuetz2023_rep1} the authors considered another option with the SAGE layer and showed that in this case the results for graphs with a degree 3 can be improved by 10.78\%.
This is reflected in the second value in the corresponding column.
Results for graphs with other $d$ are omitted since they were not published.
%We extrapolated the possible value of the architecture with SAGE layer for graphs with $d=5$ by adding 10.78\% to the results of PI-GNN with GCN layer from \cite{Schuetz2022}, and also put this \emph{P-value} in the table.
%Reproducing the results of the article \cite{Schuetz2022} caused some difficulties, so we decided to omit the \emph{P-values} for other $d$ in the table.

For QRF-GNN we estimated the \emph{P-value} on two sets of 100 graphs and noticed the negligible difference.
Therefore, the final \emph{P-value} in the table is obtained by averaging over 200 graphs.
We present results for the best value out of 5 and 15 runs for graphs with $d=3$ and the best out of 5 runs for the rest.
As one can see, QRF-GNN clearly outperforms RUN-CSP and PI-GNN in all cases and starting from $d=5$ shows the best results over all considered algorithms.
Increasing the number of runs to 15 allows QRF-GNN to show the best result on graphs with $d=3$ as well.



We also evaluated QRF-GNN on benchmark graphs from a Gset collection \cite{Gset}.
To make the evaluation more informative, we implemented $\tau$-EO heuristic from~\cite{Boettcher2001}.
As suggested by authors, we set $\tau = 1.3$ and the number of single spin updates was limited by $10^7$.
For small graphs $\tau$-EO can find a high-quality solution, but with increase of the graph size the accuracy of the algorithm degrades due to the limited number of updates.
This behavior is expected by the authors, who suggested optimal scaling for number of updates as ${\sim}O(\vert \gV \vert^3)$.
However, it is computationally expensive to carry out the required number of iterations.
We performed 20 runs of EO with different initializations to partially compensate for this.
Within the given limit, the EO algorithm took $\sim$6800 seconds per run to obtain a solution for the relatively large graph G70.








Table \ref{table:res-maxcut-gset} contains the comparison results of our algorithm with PI-GNN, RUN-CSP, EO and the SOTA heuristics Breakout Local Search (BLS) \cite{BENLIC20131162} and the Tabu Search based Hybrid Evolutionary Algorithm (TSHEA) \cite{WU2015827}.
QRF-GNN as well as BLS and TSHEA was run 20 times on each graph.
The best attempt out of 64 was chosen for RUN-CSP in original papers.
In order to obtain the results of PI-GNN, the authors applied hyperparameter optimization for each graph.
The results of RUN-CSP for the G70 graph was obtained by running the code\footnote{\url{https://github.com/toenshoff/RUN-CSP}} with parameters reported in \cite{Tonshoff2021}.

Our algorithm outperforms both neural network approaches, but it is inferior to the SOTA heuristics.
It gives the same results on graphs G49 and G50 and provides better results only for the G70 graph.
It should be noted that the solution search time for the G70 graph was $1033$~s in the case of QRF-GNN, while BLS and TSHEA took several times more, or about $11365$~s and $6932$~s correspondingly \cite{BENLIC20131162, WU2015827}.








We performed experiments on graphs from the COLOR dataset \cite{COLOR} and additional calculations for three citation graphs Cora, Citeseer and Pubmed \cite{Li2022RethinkingGN}.
Results of graph coloring with the optimal number of colors are compared with other neural network architectures, such as PI-GNN \cite{schuetz2022coloring}, GNN-1N \cite{wang2023graph} and GDN \cite{Li2022RethinkingGN}, and the SOTA heuristics HybridEA \cite{HybridEA}  (see Table \ref{table:res-coloring-conflicts}).
Missing results for PI-GNN mean that they are not contained in the source paper.
The code\footnote{\url{http://rhydlewis.eu/gcol/}} which was used for the HybridEA estimation is based on \cite{bookHybridEA}.
%We have not included results for the SOTA heuristic HybridEA here since it shows less performance than the rest, as follows from \cite{Li2022RethinkingGN}.
To evaluate the results of QRF-GNN, we did up to 10 runs for some graphs, although most of them required only one run.
It can be seen from Table \ref{table:res-coloring-conflicts} that QRF-GNN shows the best results on all instances.

%\begin{table}[t]

Table \ref{table:res-coloring-chromatic} shows the number of colors that the algorithm needs to color the graph without violations.
Results of GNN-1N and GDN were not shown in the original paper.
We also added results of RUN-CSP taken from \cite{Tonshoff2021}.

Blanked lines in Table \ref{table:res-coloring-chromatic} refer to that results have not been published.
To find the number of colors required to color the graph without violations, we successively increased the number of colors in each new run until the correct coloring was found among 10 seeds.
It is clear from Table \ref{table:res-coloring-chromatic} that QRF-GNN is superior to the presented neural network based algorithms on all considered graphs.
It is comparable to the SOTA heuristics HybridEA, and it shows the worse result only on 1 graph out of 19.
The HybridEA method works much faster on considered graphs and converges within 1~ms to 6.5~s, however, this difference becomes smaller as the graph size increases.
The convergence time for PI-GNN and QRF-GNN is shown in Table \ref{table:res-coloring-runtime}.
The number of iterationss for convergence of QRF-GNN on citation graphs was no more than 6000 and varied for the COLOR dataset from $\sim$200 to $9 \times 10^4$.
The estimated runtime for QRF-GNN turned out to be significantly less than for PI-GNN, and in some cases the difference reaches more than three orders of magnitude.
This is due to the fact that QRF-GNN does not require exhaustive tuning of hyperparameters for each instance in contrast to PI-GNN \cite{schuetz2022coloring}.




For MIS, we conduct experiments on Erdos-Renyi (ER) random graphs \cite{Erdos1984OnTE} datasets of 700-800 vertices and 9000-11000 vertices. The results are shown in \ref{table:mis}, where we compare QRF-GNN with range of
cutting edge learning-based algorithms. Supervised Learning (SL) methods: Intel \cite{Li2018CombinatorialOW},
Difusco \cite{sun2023difusco}, T2TCO \cite{li2023from}, Reinforement Learning (RL): LwD \cite{Ahn}, DIMES \cite{qiu2022dimes} and Unsupervised (UL) GflowNets \cite{zhang2023let}.
We also consider the results of SOTA MIS solver Kamis \cite{Lamm2017}, in particular ReduMIS algorithm.

The results of Kamis (ReduMIS ),  are taken from  and for are taken from \cite{qiu2022dimes}. For some of the baselines
the different results are avaliable related to the different (greedy or sampling) solution decoding.
For each such case we took the results of the best average MIS size.
Difusco is not scalable to solve large problems
from ER-9000-11000 dataset.




QRF-GNN performs the best among all learning methods. This is especially evident on large graphs, where it almost achieves the results of Kamis, being significantly superior in terms of speed.

==> reproducibility.tex <==
To ensure that the results of the article can be reproduced, we have provided the scheme of the QRF-GNN architecture and its pseudocode in section \ref{sec:rec-pi-gnn}.
A description of the main parameters and convergence criteria is contained in section \ref{sec:experiments}.
We have also included additional training details and information about utilized packages in Appendix.
It is worth noting that due to the stochastic behavior of the algorithm the results may differ depending on the initialization.
We encourage everyone to collect enough statistics by doing several independent runs to obtain high-quality results.

